CAVE: Controllable Authorship Verification Explanations

Authorship Verification (AV) (do two documents have the same author?) is essential in many real-life applications. AV is often used in privacy-sensitive domains that require an offline proprietary model that is deployed on premises, making publicly served online models (APIs) a suboptimal choice. Current offline AV models however have lower downstream utility due to limited accuracy (eg: traditional stylometry AV systems) and lack of accessible post-hoc explanations. In this work, we address the above challenges by developing a trained, offline model CAVE (Controllable Authorship Verification Explanations). CAVE generates free-text AV explanations that are controlled to be (1) accessible (uniform structure that can be decomposed into sub-explanations grounded to relevant linguistic features), and (2) easily verified for explanation-label consistency. We generate silver-standard training data grounded to the desirable linguistic features by a prompt-based method Prompt-CAVE. We then filter the data based on rationale-label consistency using a novel metric Cons-R-L. Finally, we fine-tune a small, offline model (Llama-3-8B) with this data to create our model CAVE. Results on three difficult AV datasets show that CAVE generates high quality explanations (as measured by automatic and human evaluation) as well as competitive task accuracy.

==> latex/tables/allresults.tex <==
\if 0
\begin{table*}[ht]
\centering
\resizebox{0.98\linewidth}{!}{
\begin{tabular}{cccccc}
    \toprule
    % \textbf{Method $\rightarrow$} & &  \multicolumn{4}{c}{Baselines} & \multicolumn{2}{c}{\method} \\ 
    % & & \basemodel & \baselineproduct & \filteracc & \filterall & \classic & \additive \\
    % \cmidrule(lr){3-6} \cmidrule(lr){7-8} \\
    \textbf{Dataset} & \textbf{Type} & \textbf{Model} & \textbf{Method} & \textbf{\acc} & \textbf{\cons}  \\
    \midrule
    \multirow{5}{*}{\textbf{\imdb}} & \multirow{3}{*}{Baseline} & \gptft & \chot (zero-shot prompt) & $73.6$ & N/A \\
    & & \gptft & \promptav (zero-shot) & $73.0$ & N/A \\
    & & \gptft & \method  (zero-shot) & $67.8$ & to-do \\
    % & I-O & \tfivethree & finetuned & 67.3 & N/A \\
    % & I-O & \llamath & finetuned & to-do & N/A \\
    \cmidrule{2-6}
    & \cellcolor{lviolet} & \cellcolor{lviolet}\tfivethree & \cellcolor{lviolet}\method (fine-tuned) & \cellcolor{lviolet}67.3 & \cellcolor{lviolet}0.98 \\
    & \cellcolor{lviolet}\multirow{-2}{*}{\textbf{\method}} & \cellcolor{lviolet}\llamath & \cellcolor{lviolet}\method (fine-tuned) & \cellcolor{lviolet}\textbf{74.4} & \cellcolor{lviolet}0.99 \\
    \midrule
    \multirow{5}{*}{\textbf{\blog}} & I-RO & \gptft & \chot (zero-shot) & $62.0$ & N/A \\
    & I-RO & \gptft & \promptav (zero-shot) & $62.3$ & N/A \\
    & I-RO & \gptft & \method (zero-shot) & $56.5$ & to-do \\
    % & I-O & \tfivethree & finetuned & to-do & N/A \\
    % & I-O & \llamath & finetuned & to-do & N/A \\
    \cmidrule{2-6}
    & \cellcolor{lviolet}I-RO & \cellcolor{lviolet}\tfivethree & \cellcolor{lviolet}\method (fine-tuned) & \cellcolor{lviolet}57.4 & \cellcolor{lviolet}to-do \\
    & \cellcolor{lviolet}I-RO & \cellcolor{lviolet}\llamath & \cellcolor{lviolet}\method (fine-tuned) & \cellcolor{lviolet}60.3 & \cellcolor{lviolet}to-do \\
    \midrule
    \multirow{5}{*}{\textbf{\fanfic}} & I-RO & \gptft & \chot (zero-shot) & xx & N/A \\
    & I-RO & \gptft & \promptav (zero-shot) & $xx$ & N/A \\
    & I-RO & \gptft & \method (zero-shot) & $xx$ & to-do \\
    % & I-O & \tfivethree & finetuned & to-do & N/A \\
    % & I-O & \llamath & finetuned & to-do & N/A \\
    \cmidrule{2-6}
    & \cellcolor{lviolet}I-RO & \cellcolor{lviolet}\tfivethree & \cellcolor{lviolet}\method (fine-tuned) & \cellcolor{lviolet}xx & \cellcolor{lviolet}to-do \\
    & \cellcolor{lviolet}I-RO & \cellcolor{lviolet}\llamath & \cellcolor{lviolet}\method (fine-tuned) & \cellcolor{lviolet}xx & \cellcolor{lviolet}to-do \\
    \bottomrule 
\end{tabular}
}
\caption{caption}
\label{tab:exps}
\end{table*}

\fi

% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage{graphicx}
\begin{table*}[h!]
\centering
\resizebox{\textwidth}{!}{%
% \begin{tabular}{|c|c|c|c|c|c|c|c|c|}
\begin{tabular}{ccccccccc}
\toprule
\multirow{2}{*}{Model} & \multirow{2}{*}{Method} & Test $\rightarrow$  & \multicolumn{2}{c}{\imdb} & \multicolumn{2}{c}{\blog} & \multicolumn{2}{c}{\ff} \\
\cmidrule(lr){3-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7} \cmidrule(lr){8-9}
 &  & Train $\downarrow$ & \accs & \conss & \accs & \conss & \accs & \conss \\ \midrule
\multirow{3}{*}{\gptft} & \chot & \multirow{3}{*}{Zero-shot} & 73.6 & - & 62.0 & - & 54.2 & - \\
 & \promptav &  & 73.0 & - & 62.2 & - & 57.0 & - \\
 & \method's prompt &  & 67.6 & 0.86 & 57.7 & 0.73 & 52.2 & 0.67 \\
 \midrule
  \multirow{2}{*}{\llamath} & \chot & \multirow{3}{*}{Zero-shot}  & 62.4 & - & 60.7 & - & 57.5 & - \\
   \multirow{2}{*}{\textsc{-Instruct}} & \promptav &   & 62.8 & - & 57.9 & - & 53.8 & - \\
   & \method's prompt &   & 36.7 & 0.16 & 38.8 & 0.25 & 45.5 & 0.17 \\
    \midrule
  &   &  \imdb & \cellcolor{lviolet}\textbf{75.7} & \cellcolor{lviolet}\textbf{0.97} & \cellcolor{lviolet}57.7 & \cellcolor{lviolet}\textbf{0.95} & \cellcolor{lviolet}\textbf{58.7} & \cellcolor{lviolet}\textbf{0.92} \\
 &  & \blog  & \cellcolor{lviolet}73.8 & \cellcolor{lviolet}0.93 & \cellcolor{lviolet}\textbf{60.4} & \cellcolor{lviolet}0.94 & \cellcolor{lviolet}50.6 & \cellcolor{lviolet}0.74 \\
 &  & \ff  & \cellcolor{lviolet}68.6 & \cellcolor{lviolet}0.70 & \cellcolor{lviolet}57.4 & \cellcolor{lviolet}0.83 & \cellcolor{lviolet}\textbf{60.2} & \cellcolor{lviolet}0.81 \\
  \multirow{-4}{*}{\llamath} & \multirow{-4}{*}{\textbf{\method}}  & All 3  & \cellcolor{lviolet}\textbf{74.9} & \cellcolor{lviolet}\textbf{0.99} & \cellcolor{lviolet}\textbf{57.9} & \cellcolor{lviolet}\textbf{0.96} & \cellcolor{lviolet}\textbf{58.6} & \cellcolor{lviolet}\textbf{0.91} \\
\bottomrule
\end{tabular}%
}
\caption{}
\label{tab:allres}
\end{table*}

==> latex/tables/dataset_splits.tex <==
\begin{table}[]
    \centering
    \resizebox{0.95\linewidth}{!}{
    \begin{tabular}{c|ccc}
        \hline
         Dataset & Train & Validation & Test \\ \hline
        \imdb & & & \\
        \blog & & & \\
        \ff & & & \\ \hline
    \end{tabular}}
    \caption{Dataset split details}
    \label{tab:splits}
\end{table}

==> latex/tables/prompt.tex <==
\begin{table*}[h!]
    \centering
    \small
    \begin{tabular}{p{0.95\textwidth}}
    \toprule
    \textbf{\method's Prompt:} \\
    Task: On a scale of 0 to 1, with 0 indicating low confidence and 1 indicating high confidence, please provide a general assessment of the likelihood that Text 1 and Text 2 were written by the same author. Your answer should reflect a moderate level of strictness in scoring. Here are some relevant variables to this problem. \\
    1. punctuation style (e.g. hyphen, brackets, colon, comma, parenthesis, quotation mark) \\
    2. special characters style, capitalization style (e.g. Continuous capitalization, capitalizing certain words) \\
    3. acronyms and abbreviations(e.g. Usage of acronyms such as OMG, Abbreviations without punctuation marks such as Mr Rochester vs. Mr. Rochester,Unusual abbreviations such as def vs. definitely) \\
    4. writing style \\
    5. expressions and Idioms \\
    6. tone and mood \\
    7. sentence structure \\
    8. any other relevant aspect \\
    \hl{Provide the answer in a Python JSON format. Use the following keys for your dictionary: `punctuation style', `special characters style, capitalization style', `acronyms and abbreviations', `writing style', `expressions and Idioms', `tone and mood', `sentence structure', `any other relevant aspect', `final score'. Apart from the `final score', everything else must have a text value; also, the text should include a concluding YES/NO/MAYBE about whether the two texts are similar or not with respect to the key at hand. Finally, provide an `output' key in your dictionary, which says YES if the two texts are written by the same author, and NO otherwise.}\\\\
    Text1: excellent until a completely unsatisfying ending This movie really got me hooked. The plot about... \\\\
    Text2: A Nutshell Review: Oliver Twist ``Please sir, may I have some more?'' Ah, the immortal line from... \\
    \bottomrule
    \end{tabular}
    \caption{Our prompt is inspired from \cite{promptav} (the non-highlighted part). We add the instructions in the highlighted part to prompt the output to be in a python dictionary format, so as to improve controllability in terms of the structure/parsing of the output and automatic verification of the consistency between the rationale and the label.}
    \label{tab:prompt}

    % \begin{tabular}{p{0.95\textwidth}}
    % \toprule
    % \textbf{\method's Output Format:} \\
    % \{ \\
    % \hl{punctuation style}: Both texts use a variety of punctuation, including commas, periods, and quotation marks, but Text 1 uses more diverse punctuation such as parentheses and hyphens. \colorbox{yellow}{\underline{MAYBE}} \\
    % \hl{special characters style, capitalization style}: Text 1 uses continuous capitalization for emphasis (e.g., 'WONDERFUL', 'THRILLED'), which is not observed in Text 2. \colorbox{yellow}{\underline{NO}}, \\
    % \hl{acronyms and abbreviations}: Neither text makes significant use of acronyms or unusual abbreviations, maintaining a formal tone. Conclusion: \colorbox{yellow}{\underline{YES}}, \\
    % \hl{writing style}: Text 1 has a more personal, reflective style, sharing personal opinions and feelings about the movie. Text 2 provides a more detached, narrative-style review without personal input. \colorbox{yellow}{\underline{NO}}, \\
    % \hl{expressions and idioms}: Both texts avoid colloquial expressions and idioms, opting for a more formal review format. \colorbox{yellow}{\underline{YES}}, \\
    % \hl{tone and mood}: Text 1 has a more varied tone, from enthusiasm to disappointment, while Text 2 maintains a consistent, somewhat formal and analytical tone. \colorbox{yellow}{\underline{NO}}, \\
    % \hl{sentence structure}: Text 1 features a mix of short and long sentences with more complex structures, while Text 2 tends to use more uniformly structured, intermediate-length sentences. \colorbox{yellow}{\underline{MAYBE}}, \\
    % \hl{any other relevant aspect}: The approach to movie critique is different; Text 1 is more about the impact on the viewer, while Text 2 focuses on plot summary and cinematic elements. \colorbox{yellow}{\underline{NO}}, \\
    % \hl{final score}: \colorbox{yellow}{\underline{0.375}}, \\
    % \hl{output}: \colorbox{yellow}{\underline{NO}} \\
    % \} \\
    % \bottomrule
    % \end{tabular}
    % \caption{This table represents a sample output by \method, with the rationale and the output in a Python dictionary format. The text (dictionary keys) highlighted in blue depict the various linguistic features considered for getting an \av explanation, as well as the keys for final confidence score and predicted task output. The text underlined and highlighted in yellow depict the intermediate labels with respect to each linguistic feature, the confidence score value, and the predicted task label. We use the predicted label to measure task \acc and all of them to measure \cons between the explanation and the label.}
    % \label{tab:dict}    
\end{table*}




==> latex/tables/results.tex <==
\if 0
\begin{table*}[ht]
\centering
\resizebox{0.98\linewidth}{!}{
\begin{tabular}{cccccc}
    \toprule
    % \textbf{Method $\rightarrow$} & &  \multicolumn{4}{c}{Baselines} & \multicolumn{2}{c}{\method} \\ 
    % & & \basemodel & \baselineproduct & \filteracc & \filterall & \classic & \additive \\
    % \cmidrule(lr){3-6} \cmidrule(lr){7-8} \\
    \textbf{Dataset} & \textbf{Type} & \textbf{Model} & \textbf{Method} & \textbf{\acc} & \textbf{\cons}  \\
    \midrule
    \multirow{5}{*}{\textbf{\imdb}} & \multirow{3}{*}{Baseline} & \gptft & \chot (zero-shot prompt) & $73.6$ & N/A \\
    & & \gptft & \promptav (zero-shot) & $73.0$ & N/A \\
    & & \gptft & \method  (zero-shot) & $67.8$ & to-do \\
    % & I-O & \tfivethree & finetuned & 67.3 & N/A \\
    % & I-O & \llamath & finetuned & to-do & N/A \\
    \cmidrule{2-6}
    & \cellcolor{lviolet} & \cellcolor{lviolet}\tfivethree & \cellcolor{lviolet}\method (fine-tuned) & \cellcolor{lviolet}67.3 & \cellcolor{lviolet}0.98 \\
    & \cellcolor{lviolet}\multirow{-2}{*}{\textbf{\method}} & \cellcolor{lviolet}\llamath & \cellcolor{lviolet}\method (fine-tuned) & \cellcolor{lviolet}\textbf{74.4} & \cellcolor{lviolet}0.99 \\
    \midrule
    \multirow{5}{*}{\textbf{\blog}} & I-RO & \gptft & \chot (zero-shot) & $62.0$ & N/A \\
    & I-RO & \gptft & \promptav (zero-shot) & $62.3$ & N/A \\
    & I-RO & \gptft & \method (zero-shot) & $56.5$ & to-do \\
    % & I-O & \tfivethree & finetuned & to-do & N/A \\
    % & I-O & \llamath & finetuned & to-do & N/A \\
    \cmidrule{2-6}
    & \cellcolor{lviolet}I-RO & \cellcolor{lviolet}\tfivethree & \cellcolor{lviolet}\method (fine-tuned) & \cellcolor{lviolet}57.4 & \cellcolor{lviolet}to-do \\
    & \cellcolor{lviolet}I-RO & \cellcolor{lviolet}\llamath & \cellcolor{lviolet}\method (fine-tuned) & \cellcolor{lviolet}60.3 & \cellcolor{lviolet}to-do \\
    \midrule
    \multirow{5}{*}{\textbf{\fanfic}} & I-RO & \gptft & \chot (zero-shot) & xx & N/A \\
    & I-RO & \gptft & \promptav (zero-shot) & $xx$ & N/A \\
    & I-RO & \gptft & \method (zero-shot) & $xx$ & to-do \\
    % & I-O & \tfivethree & finetuned & to-do & N/A \\
    % & I-O & \llamath & finetuned & to-do & N/A \\
    \cmidrule{2-6}
    & \cellcolor{lviolet}I-RO & \cellcolor{lviolet}\tfivethree & \cellcolor{lviolet}\method (fine-tuned) & \cellcolor{lviolet}xx & \cellcolor{lviolet}to-do \\
    & \cellcolor{lviolet}I-RO & \cellcolor{lviolet}\llamath & \cellcolor{lviolet}\method (fine-tuned) & \cellcolor{lviolet}xx & \cellcolor{lviolet}to-do \\
    \bottomrule 
\end{tabular}
}
\caption{caption}
\label{tab:exps}
\end{table*}

\fi

% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage{graphicx}
\begin{table*}[h!]
\centering
\resizebox{\textwidth}{!}{%
% \begin{tabular}{|c|c|c|c|c|c|c|c|c|}
\begin{tabular}{ccccccccc}
\toprule
\multirow{2}{*}{Model} & \multirow{2}{*}{Method} & Test $\rightarrow$  & \multicolumn{2}{c}{\imdb} & \multicolumn{2}{c}{\blog} & \multicolumn{2}{c}{\ff} \\
\cmidrule(lr){3-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7} \cmidrule(lr){8-9}
 &  & Train $\downarrow$ & \accs & \conss & \accs & \conss & \accs & \conss \\ \midrule
 \textsc{SVM} & - & Single-dataset & 59.7 & - & 56.2 & - & 55.7 & - \\ \midrule
\multirow{4}{*}{\gptft} & \chot & Zero-shot & 73.6 & - & 62.0 & - & 54.2 & - \\
 & \promptav & Zero-shot & 73.0 & - & 62.2 & - & 57.0 & - \\
 & \method's prompt & Zero-shot & 67.6 & 0.86 & 57.7 & 0.73 & 52.2 & 0.67 \\
 & \method's prompt & Few-shot & 71.3 & 0.94 & 64.0 & 0.97* & 61.7* & 0.86  \\
 \midrule
   & \chot & Zero-shot  & 62.4 & - & 60.7 & - & 57.5 & - \\
   \llamath & \promptav &  Zero-shot & 62.8 & - & 57.9 & - & 53.8 & - \\
   \textsc{-Instruct} & \method's prompt &  Zero-shot & 36.7 & 0.16 & 38.8 & 0.25 & 45.5 & 0.17 \\
   & \method's prompt & Few-shot & 53.8 & 0.98 & 62.3 & 0.99 & 48.1 & 0.93  \\ 
    \midrule
    % 1280
    \multirow{4}{*}{\llamath} & \multirow{2}{*}{\chot} & Single-dataset & 65.7 & - & 64.6 & - & 60.5 & - \\
    & & Multi-dataset & 65.3 & - & 65.0 & - & 61.5 & - \\  \cmidrule(lr){2-9}
    & \multirow{2}{*}{\promptav} & Single-dataset & 76.2 & - & 61.3 & - & xx & - \\
    & & Multi-dataset & 76.0 & - & 63.8 & - & 60.8 & - \\ \midrule \midrule 
   \multirow{2}{*}{\llamath} & \method (all ling- & Single-dataset & \cellcolor{lviolet}74.1 & \cellcolor{lviolet}0.99 & \cellcolor{lviolet}60.6 & \cellcolor{lviolet}1.00 & \cellcolor{lviolet}62.6 & \cellcolor{lviolet}0.99 \\ 
      & -uistic features)  & Multi-dataset  & \cellcolor{lgreen}\textbf{73.2} & \cellcolor{lgreen}\textbf{1.00} & \cellcolor{lgreen}\textbf{58.4} & \cellcolor{lgreen}\textbf{0.99} & \cellcolor{lgreen}\textbf{59.6} & \cellcolor{lgreen}\textbf{0.99} \\ \midrule 
      \multirow{2}{*}{\llamath} & \method (remove & Single-dataset & \cellcolor{lviolet}73.5 & \cellcolor{lviolet}0.99 & \cellcolor{lviolet}55.3 & \cellcolor{lviolet}0.95 & \cellcolor{lviolet}61.7 & \cellcolor{lviolet}0.98 \\ 
      & least useful feature)  & Multi-dataset  & \cellcolor{lgreen}\textbf{73.6} & \cellcolor{lgreen}\textbf{0.99} & \cellcolor{lgreen}\textbf{57.0} & \cellcolor{lgreen}\textbf{1.0} & \cellcolor{lgreen}\textbf{60.2} & \cellcolor{lgreen}\textbf{0.99} \\ \midrule 
      \multirow{2}{*}{\llamath} & \method (remove 2 & Single-dataset & \cellcolor{lviolet}70.6 & \cellcolor{lviolet}0.99 & \cellcolor{lviolet}56.4 & \cellcolor{lviolet}0.97 & \cellcolor{lviolet}60.9 & \cellcolor{lviolet}0.98 \\ 
      & least useful features)  & Multi-dataset  & \cellcolor{lgreen}\textbf{75.2} & \cellcolor{lgreen}\textbf{0.99} & \cellcolor{lgreen}\textbf{58.0} & \cellcolor{lgreen}\textbf{1.0} & \cellcolor{lgreen}\textbf{61.0} & \cellcolor{lgreen}\textbf{0.99} \\ %\midrule  \midrule \midrule  \midrule 
   % \multirow{2}{*}{\llamath} & \method (all ling- & Single-dataset & \cellcolor{lviolet}73.5 & \cellcolor{lviolet}0.99 & \cellcolor{lviolet}59.8 & \cellcolor{lviolet}0.98 & \cellcolor{lviolet}61.0 & \cellcolor{lviolet}0.92 \\ 
   %    & -uistic features)  & Multi-dataset  & \cellcolor{lgreen}\textbf{xx} & \cellcolor{lgreen}\textbf{x} & \cellcolor{lgreen}\textbf{xx} & \cellcolor{lgreen}\textbf{xx} & \cellcolor{lgreen}\textbf{xx} & \cellcolor{lgreen}\textbf{xx} \\ \midrule 
   %    \multirow{2}{*}{\llamath} & \method (remove  & Single-dataset & \cellcolor{lviolet}xx & \cellcolor{lviolet}xx & \cellcolor{lviolet}xx & \cellcolor{lviolet}xx & \cellcolor{lviolet}xx & \cellcolor{lviolet}xx \\ 
   %    & least useful feature)  & Multi-dataset  & \cellcolor{lgreen}\textbf{73.2} & \cellcolor{lgreen}\textbf{0.99} & \cellcolor{lgreen}\textbf{58.2} & \cellcolor{lgreen}\textbf{0.99} & \cellcolor{lgreen}\textbf{60.0} & \cellcolor{lgreen}\textbf{0.99} \\ \midrule
   %    \multirow{2}{*}{\llamath} & \method (remove 2 & Single-dataset & \cellcolor{lviolet}70.7 & \cellcolor{lviolet}0.99 & \cellcolor{lviolet}57.6 & \cellcolor{lviolet}0.93 & \cellcolor{lviolet}xx & \cellcolor{lviolet}xx \\ 
   %    & least useful features)  & Multi-dataset  & \cellcolor{lgreen}\textbf{76.1} & \cellcolor{lgreen}\textbf{0.98} & \cellcolor{lgreen}\textbf{58.5} & \cellcolor{lgreen}\textbf{0.99} & \cellcolor{lgreen}\textbf{61.8} & \cellcolor{lgreen}\textbf{0.98} \\ \midrule  \midrule \midrule \midrule  
      % 768
   %  \multirow{4}{*}{\llamath} & \multirow{2}{*}{\chot} & Single-dataset & 62.0 & - & 64.2* & - & 61.5 & - \\
   %  & & Multi-dataset & 75.3 & - & 62.5 & - & 57.6 & - \\  \cmidrule(lr){2-9}
   %  & \multirow{2}{*}{\promptav} & Single-dataset & 63.8 & - & 58.4 & - & 58.2 & - \\
   %  & & Multi-dataset & 68.6 & - & 62.7 & - & 63.3 & - \\ \midrule \midrule 
   % \multirow{2}{*}{\llamath} & \multirow{2}{*}{\method} & Single-dataset & \cellcolor{lviolet}75.7* & \cellcolor{lviolet}0.97 & \cellcolor{lviolet}60.4 & \cellcolor{lviolet}0.94 & \cellcolor{lviolet}60.2 & \cellcolor{lviolet}0.81 \\ 
   %    &  & Multi-dataset  & \cellcolor{lgreen}\textbf{74.9} & \cellcolor{lgreen}\textbf{0.99}* & \cellcolor{lgreen}\textbf{57.9} & \cellcolor{lgreen}\textbf{0.96} & \cellcolor{lgreen}\textbf{58.6} & \cellcolor{lgreen}\textbf{0.91}* \\
\bottomrule
\end{tabular}%
}
\caption{Empirical Results comparing baselines and \method. We note that both single dataset and multi-dataset trained models beat/are competitive with strong baselines such as \gptft. Note that the single-dataset results each correspond to three different \method models trained on the respective training sets.}
\label{tab:exps}
\end{table*}
